High Fidelity Speech Synthesis with Adversarial Networks

Generative adversarial networks have seen rapid development in recent years and have led to remarkable improvements in generative modelling of images. However, their application in the audio domain has received limited attention, and autoregressive models, such as WaveNet, remain the state of the art in generative modelling of audio signals such as human speech. To address this paucity, we introduce GAN-TTS, a Generative Adversarial Network for Text-to-Speech. Our architecture is composed of a conditional feed-forward generator producing raw speech audio, and an ensemble of discriminators which operate on random windows of different sizes. The discriminators analyse the audio both in terms of general realism, as well as how well the audio corresponds to the utterance that should be pronounced. To measure the performance of GAN-TTS, we employ both subjective human evaluation (MOS - Mean Opinion Score), as well as novel quantitative metrics (Fr\'echet DeepSpeech Distance and Kernel DeepSpeech Distance), which we find to be well correlated with MOS. We show that GAN-TTS is capable of generating high-fidelity speech with naturalness comparable to the state-of-the-art models, and unlike autoregressive models, it is highly parallelisable thanks to an efficient feed-forward generator. Listen to GAN-TTS reading this abstract at https://storage.googleapis.com/deepmind-media/research/abstract.wav.

==> old_model.tex <==
\section{\acronym}\label{s:model}
\karen{I think we only need Generator and Discriminators subsections. Can also have Data section which would be 5.1 Datasets section and conditioning}
In this section we present the architecture of the proposed model. We describe the main components of our model: two variants of \emph{Random Window Discriminators} ({\rwd}s) and dilated residual blocks.
\karen{not sure we want to highlight dilated blocks that explicitly, they've been used before}
We also elaborate on the way the linguistic features are processed through a model. Finally, we present details of the architectures of the Generator and the Discriminators, and construction of their ensemble.

\subsection{Random Window Discriminators}\label{s:rwds}
\karen{this section should be merged into the discriminator section}
We consider {\rwd}s, which operate on randomly sub-sampled fragments of the real or generated samples. %\karen{ablate random window}
Random Window Discriminators allow us to discriminate between lower-dimensional distributions, at the same time giving access to a larger number of real samples.

We use multiple discriminators with different window lengths. 
However, in the first layer we downsample \footnote{Downsampling is done by reshaping the signal which moves consecutive blocks of samples into the channel dimension, i.e.\ from $[Tk,1]$ to $[T,k]$, where $T$ is the window length after downsampling and $k$ is the downsampling factor.} 
by a factor proportional to the window size, effectively allowing discriminators to work on different frequencies, at the same time keeping similar structure of different discriminators.

We consider both conditional and unconditional discriminators.
The latter do not see the conditioning that corresponds to the sampled window, hence could not be used on their own, and should be used in combination with conditional discriminators. On the other hand, random windows in conditional discriminators need to be aligned with the conditioning frequency to preserve correspondence between waveform and linguistic features within the sampled window. One step in the conditioning corresponds to 5ms, or 120 steps of waveform, hence such sampling is constrained by a 120 times lower frequency.
Unconditional discriminators are free of such constraints and thus are exposed to even richer samples from real and generated distributions.
\input{tables/generator.tex}
\input{figs/discriminator.tex}

\subsection{Conditioning}\label{s:conditioning}
\karen{this section should be split and merged into generator and discriminator sections.}
We train models conditional on linguistic features and the speaker number (in the multi-speaker case). Linguistic features that we use are similar to those used in WaveNet~\citep{wavenet}; they encode information such as phoneme as well as logarithmic fundamental frequency $\log F_0$ and are computed for 5ms windows (frequency of 200Hz). In total, there are 568 features. 
Since such conditioning has temporal structure, we use it as an input to the very first layer of the generator and keep the temporal dimension at each of the following layers. We gradually upsample the hidden representations in between the convolutional layers to account for the ratio of the frequencies of the conditioning and raw audio.

As mentioned above, we use multiple {\rwd}s, half of which are conditional, half are not. In conditional ones, aligned random windows are sub-sampled from a waveform and its corresponding conditioning. The waveform fragment is passed through the convolutional stack which gradually downsamples the temporal dimension of following hidden units, until it is equal to that of the conditioning, at which point both are concatenated. This joint information is then passed to remaining blocks whose final output is average-pooled and a scalar output is returned.
\input{figs/blocks.tex}

\subsection{Dilated residual blocks}\label{s:blocks}
\karen{this section should be split and merged into generator and discriminator sections.}
As in raw audio modelling we normally deal with long sequences, we needed to ensure that the receptive fields of our networks will be able to learn dependencies at various frequencies, including long- and short-term ones. For that reason, we build our networks using stacks of residual blocks with dilated convolutions. 

Figure \ref{f:blocks} shows details of the blocks used in the model. In discriminators, we use dilation factors one and two in two main convolutions forming a residual block. Additional two $1\times 1$ convolutions are used in a skip connection and for embedding of the conditioning, which is added to the hidden representation after the first layer. The number of channels doubles in each block immediately after downsampling, which is applied at the very beginning on both hidden representation and linguistic features.

We build generator $\g$ using dilated residual blocks, detailed in Fig. \ref{f:gblock}. Each block contains four main convolutions with doubling dilation factors, from 1 to 8. Convolutions are followed by Conditional BatchNorms \citep{cond-batch-norm}, conditioned on the linear embeddings (separate for each BatchNorm instance) of the noise term $z\sim\mathcal{N}(0,\mI_{128})$ in the single-speaker case or the concatenation of $z$ and one-hot representation of the speaker number in the multi-speaker case. The block contains two skip connections, the first of which uses $1\times 1$ \emph{convolution}.

\subsection{Generator architecture}
We use seven blocks described above in $\g$. Blocks 3-7 additionally halve the number of output channels in their first convolutions and upsample the hidden representations respectively by factors of $2,2,2,3,5$. Overall, residual blocks upsample the input's temporal dimension of $400$ to $48000$, i.e. the length of 2 seconds of audio at 24kHz. The final convolutional layer with \emph{Tanh} activation produces a single channel audio waveform.

A summary of $\g$'s architecture is presented in Table \ref{t:generator}.

\subsection{Discriminator architectures}
Our \emph{base} discriminators are comprised of the residual blocks described in Section \ref{s:blocks}. First and the last two blocks do not downsample (i.e. keep the temporal dimension fixed). Apart from that, we add at least two downsampling blocks in the middle, with downsample factors depending on $k$. Details are presented in Appendix \ref{a:discriminator-details}.

By $\cd_k$ and $\ud_k$ we will denote conditional and unconditional discriminators, respectively. In $\cd_k$,  the last downsampling block is conditional as shown in Fig. \ref{f:cdblock}; all other blocks used in $\cd_k$ and $\ud_k$ are unconditional, as in Fig. \ref{f:dblock}.
Both of these discriminators have fully convolutional architectures.

We define conditional and unconditional \emph{Random Window Discriminators} as stochastic functions 
\begin{align}
    \crwd_{k, \omega}(x, c; \theta) &= \cd_k(x_{\rj:\rj + \omega k}, c_{\rj/\lambda: (\rj + \omega k)/\lambda}; \theta),\qquad \rj\sim\mathcal{U}\left(\left\{0,\lambda, 2\lambda,\ldots,N - \omega k\right\}\right) \\
    \urwd_{k, \omega}(x; \theta) &= \ud_k(x_{\rj:\rj + \omega k}; \theta),\qquad \rj\sim\mathcal{U}\left(\left\{0,1,\ldots,N -\omega k\right\}\right),
\end{align}
where $\omega$ is the base window size\footnote{\emph{Base windows size} $\omega$ is the window size \emph{after} the strided convolution; the corresponding effective window size is $\omega k$.}, $x$ and $c$ are respectively the waveform and linguistic features, $\theta$ is set of network parameters, and $\lambda=120$ is a frequency ratio between $x$ and $c$.\footnote{We assume that $\lambda$ is an integer that evenly divides $N - \omega k$.\sander{Shouldn't this footnote be the other way around, it's omega that should be a multiple of lambda since lambda is fixed (we did not get to choose it)}}

The proposed discriminator combines 10 different {\rwd}'s:
\begin{equation}
    \mathsf{mRWD}^*_{\omega}(x, c; \theta^*) = \sum_{k\in\{1,2,4,8,15\}}\crwd_{k, \omega}(x, c; \theta_k) + \urwd_{k, \omega}(x; \theta_k'), \qquad \theta^* = \bigcup_k(\theta_k \cup \theta_k').
\end{equation}
In Section \ref{s:experiments} we describe other combinations of {\rwd}s as well as a full, deterministic discriminator which we used in our ablation study.

For brevity, we will often skip $\omega$, setting its value to 480. \sander{This sentence looks a bit lost -- if I understand correctly the point is to say that we don't vary omega in the ablation studies, but instead keep it fixed at 480? Maybe it's better to say that where the ablations are descried.}

